Time-Bin CKA as a tool for blockchain technology

We explore the potential of Time-Bin Conference Key Agreement (TB CKA) protocol as a means to achieve consensus among multiple parties. We provide an explanation of the underlying physical implementation, i.e. TB CKA fundamentals and illustrate how this process can be seen as a natural realization of the global common coin primitive. Next, we present how TB CKA could be embodied in classical consensus algorithms to create hybrid classical-quantum solutions to the Byzantine Agreement problem.

==> archive/separate-text-inputs/CKAforQB-2-1.tex <==
\subsection*{Quantum Conference Key Agreement}

\begin{figure}[b!]
\centering
\includegraphics[width=0.5\linewidth]{pic/ckaid.jpg}
\caption{The idea of four node network, connected with quantum and classical channels, in which the consensus mechanism can be obtained using CKA protocol.}
\label{fig:ckaid}
\end{figure}

Quantum Conference Key Agreement is a protocol that enables the multiparty quantum key exchange \cite{CKAthesis}. It means that the same quantum key is established between many parties. Thanks to this it is possible to  in a multiparty system.\\

The infrastructure that allows to achieve such consensus consists of two parts. One is a classical Internet cloud that connects all parties using classical communication in classical channels, the other is a quantum server that is responsible for preparing and distributing shared qubits between all parties at once. The scheme of such infrastructure is presented in Fig. \ref{fig:ckaid}. \\

\newpage
CKA is based on sharing N qubits with N communicating parties. These qubits are in specific entangled state called $|GHZ\rangle$.
The CKA protocol was experimentally demonstrated in a scheme with 4 node network in 2021 \cite{Proietti2021}. The experimental setup is presented in Figure \ref{fig:cka}. \\
As it can be seen, the nodes are connected to the quantum server. they are also connected with each other by classical channels, which is not presented in the figure. \\

The quantum server is responsible for distribution of an entangled state, which is here in a form
\begin{equation*}
|GHZ\rangle=\frac{1}{\sqrt{2}}\Big(|0000\rangle+|1111\rangle \Big) \; .
\end{equation*}
Here such quantum state is generated using two SPDC sources in Sagnac mode. The single PPLN crystal, pumped by pulsed Ti:Sapphire laser generates quantum state that can be written in a form of 
\begin{equation}
|\psi\rangle=\frac{1}{\sqrt{2}}\big(|0\rangle+|1\rangle\big) \; ,
\end{equation}  
where $|0\rangle$ and $|1\rangle$ are orthogonal polarization states. Generated qubits are correlated with each other using PBS (polarization beamsplitter) and distributed using long single-mode fibers. Then, each node measures its qubit similarly to the method used for standard BB84 protocol (collecting detections for different settings of quarter and half waveplates). \\

\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{pic/ckaexp}
\caption{Experimental setup of CKA for 4-node network. Symbols: BS -- beamsplitter, PBS -- polarization beamsplitter, PFC -- polarization controller, DM -- dichroic mirror, HWP -- half-wave plate, QWP -- quarter-wave plate, IF -- interference filter, FC -- fiber coupler, SNSPD -- superconducting nanowire single photon detector. The figure is taken from Ref. \cite{Proietti2021}. }
\label{fig:cka}
\end{figure}



On the one hand, although the experimental realization was presented only for 4 nodes separated from each other by 20 km at maximum, due to the scalability of this method, it is a promising solution worth to consider in further development of quantum consensus mechanism in distributed systems. On the other hand, due to decoherence, encoding information in the means of photon polarization state is not the best choice for long-range communication using optical fiber links. Therefore, other implementation of CKA protocol should be addressed.\\

\subsection*{Time-bin CKA}

\begin{figure}[t!]
\centering
\includegraphics[width=0.55\linewidth]{pic/tbe.jpg}
\caption{Scheme of time-bin encoding. Early- and late- time-bin in relation to the external clock.}
\label{pic:tbe}
\end{figure}

One of them could be use of time-bin encoding. Such qubits may be simply created by single photons traveling paths of different lengths. As a result, photons' arrival time, compared to external clock, differ and may be assigned as the early- and late-time-bin, as presented in Figure \ref{pic:tbe}. \\

Figure \ref{pic:ckatb} shows the proposal of experimental setup that enables to introduce CKA protocol with time-bin encoding for four node network. \\
Let us follow beam path inside the setup. 
At the beginning beam  from pulsed pump laser (PL) enters a set of beamsplitters and mirrors, resulting in creation of time bins, that may be denoted as "states" $|0\rangle$ and $|1\rangle$ (\textcolor{dg}{\textbf{dark green}} line). Then, the beam is focused on first SPDC nonlinear crystal (SPDC1), which creates a polarization qubit in a form 
\begin{equation}
|\phi\rangle=\frac{1}{\sqrt{2}}\big(|\udarr\rangle+|\lrarr\rangle\big)\; ,
\end{equation}
where $|\udarr\rangle$, $|\lrarr\rangle$ are vertical and horizontal polarization states, respectively. Taking into account previously created time bins, at this point the photon state from the beam (marked with \textcolor{lg}{\textbf{light green}} line) can be described as
\begin{equation}
|\Phi\rangle=\frac{1}{\sqrt{2}}\big(|0_{\udarr}0_{\lrarr}\rangle+|1_{\udarr}1_{\lrarr}\rangle\big)\;.
\end{equation}
Later, \textcolor{lg}{\textbf{light green}} photon beam incidents onto polarization beamsplitter (PBS), that divides the  beam into two, that are used to build the Sagnac single-photon source (in which beams pass through the crystal in opposite directions simultaneously). Let us assume that in described case beam with horizontal polarization ($\lrarr$) passes through PBS. Then, this beam is focused into the second nonlinear crystal (SPDC2), where another pair of orthogonally polarized photons are generated, so the \textcolor{lg}{\textbf{light green}} beam here is converted into \textcolor{or}{\textbf{orange}} one in such a way:
\begin{equation}
\big(|0_{\lrarr}\rangle+|1_{\lrarr}\rangle\big) \; \larr \; \big(|0_{\udarr}0_{\lrarr}\rangle+|1_{\udarr}1_{\lrarr}\rangle\big) \; .
\end{equation}
Then, the \textcolor{or}{\textbf{orange}} beam passes through half-wave plate that rotates the polarization state of each photon, resulting in a similar state $\big(|0_{\lrarr}0_{\udarr}\rangle +|1_{\lrarr}1_{\udarr}\rangle\big)$ . This photon beam is then separated by the dichroic mirror (DM), passes through another PBS and are detected in detectors D1 and D2. \\
In the other arm, beam with vertical polarization ($\udarr$) is reflected from PBS, and passes through HWP that changes its polarization to horizontal one ($\lrarr$). It enables to convert photon beam (\textcolor{lg}{\textbf{light green}} line) in the same manner for both beams that create the Sagnac source arms, resulting in a state  $\big(|0_{\lrarr}0_{\udarr}\rangle+|1_{\lrarr}1_{\udarr}\rangle\big)$ (\textcolor{or}{\textbf{orange}} line). Later, the beams that differ with polarization are separated in PBS and detected in D3 and D4. \\
It should be noted here that lines with different colors mark each state of beam conversion (wavelength change). \\

\begin{figure}[t!]
\centering
\includegraphics[width=0.85\linewidth]{pic/ckaexpset.png}
\caption{Proposal of the experimental setup for implementation of time-bin CKA protocol. Symbols: PL -- pulsed laser, BS -- beamsplitter, M --mirror, L -- lens, F -- filter, DM -- dichroic mirror, PBS -- polarization beamsplitter, SPDC1, SPDC2 -- nonlinear crystals, D1,D2,D3,D4 -- single-photon detectors. Converted photon beams are marked with different color lines.}
\label{pic:ckatb}
\end{figure}

Finally, taking into account both conversion processes, the overall photon state before the measurement can be written as
\begin{equation}
|\Psi\rangle=\frac{1}{\sqrt{2}}\big(|0_{\lrarr}0_{\udarr}0_{\lrarr}0_{\udarr}\rangle+|1_{\lrarr}1_{\udarr}1_{\lrarr}1_{\udarr}\rangle\big) \; .
\end{equation}
Such photon state shows so-called hyperentanglement, where in correlation between photons various properties (degrees of freedom) are engaged. \\

Let us also check the kind of photon state that are prepared for detection by respective detectors:
\begin{equation}
\begin{split}
D1:& \; \; |0_{\lrarr}\rangle+|1_{\lrarr}\rangle \;,\\
D2:& \; \; |0_{\udarr}\rangle+|1_{\udarr}\rangle\;,\\
D3:& \; \; |0_{\lrarr}\rangle+|1_{\lrarr}\rangle\;,\\
D4:& \; \; |0_{\udarr}\rangle+|1_{\udarr}\rangle\;.
\end{split}
\end{equation}

Since single-photon detectors are not usually sensitive to the photon polarization state (they are more sensitive to photon wavelength), it may be concluded that in all detectors the same shared time-bin qubit is measured. Thanks to this it is possible to establish the key simultaneously with all four nodes.\\









==> archive/separate-text-inputs/CKAforQB-bib.tex <==
\section{Bibliography}
\begingroup
\small
\renewcommand{\section}[2]{}%
%\renewcommand{\chapter}[2]{}% for other classes
\begin{thebibliography}{}
\bibitem{Sun2019}{
X. Sun, M. Sopek, P. Kulicki,\textit{
Towards Quantum-Secured Permissioned Blockchain: Signature, Consensus, and Logic}, Entropy \textbf{21}(9), 887 (2019).
}
\bibitem{Wang2020}{
Q. Wang, J. Huang, S. Wang, Y. Chen, P. Zhang, L. He, \textit{A Comparative Study of Blockchain Consensus Algorithms}, J. Phys.: Conf. Ser. \textbf{1437}, 012007 (2020).
}
\bibitem{book:Wattenhofer}{
R. Wattenhofer, \textit{Distributed Ledger Technology. The Science of the Blockchain}, Createspace Independent Publishing Platform, revised 2017.
}
\bibitem{Hondt2004}{
E. D'Hondt, P. Pamamgaden, \textit{The Computational Power of the W and GHZ states}, Journ. Quantum Inf. and Comp. \textbf{6}(2), 173 (2005).
}
\bibitem{FLP}{
M.J. Fischer, N.A. Lynch, M.S. Paterson, \textit{Impossibility of Distributed Consensus with One Faulty Process}, Journal of the ACM \textbf{32}(2), 374 (1985).
}
\bibitem{Gilbert2012}{
S. Gilbert, N.A. Lynch, \textit{Perspectives on the CAP Theorem}, Computer \textbf{45}(2), 30 (2012).
}
\bibitem{Marcozzi2021}{
M. Marcozzi, L. Mostarda, \textit{Quantum Consensus: an overview}, arXiv: 2101.04192 (2021).
}
\bibitem{Proietti2021}{
M. Proietti, J. Ho, F. Grasselli, P. Barrow, M. Malik, A. Fedrizzi, \textit{Experimental quantum conference key agreement}, Sci. Adv. \textbf{7}, 23 (2021).
}
\bibitem{CKAthesis}{
F. Grasselli, \textit{Quantum Cryptography: from Key Distribution to Conference Key Agreement}, PhD thesis from the Institute for Theoretical Physics III at the Heinrich-Heine-Universität Düsseldorf (2020).
}
\bibitem{Grasselli2019}{
F. Grasselli, H. Kampermann, D. Bruss, \textit{Conference key agreement with single-photon interference}, New J. Phys \textbf{21}, 123002 (2019).
}
\bibitem{Wooters1982}{
W. Wootters, W. Zurek, \textit{A Single Quantum Cannot be Cloned}, Nature \textbf{299}(5886), 802 (1982).
}
\bibitem{BB84}{
C.H.~Bennett, G.~Brassard, \textit{Quantum cryptography: Public key distribution and coin tossing},  Proc. of IEEE Int. Conf. on Computers, Systems and Signal Processing \textbf{175}, 8 (1984).
}

\bibitem{Sopek2022}{
M. Sopek, D. Tomaszuk, Sz. Głąb, F. Turoboś, I. Zieliński, D. Kuziński, R. Olejnik, P. Łuniewski and P. Grądzki, \textit{Technological Foundations of Ontological Ecosystems on the 3rd Generation Blockchains}, IEEE Access, vol. 10, pp. 12487-12502, 2022, doi:10.1109/ACCESS.2022.3141014.}  

\end{thebibliography}


==> archive/separate-text-inputs/CKAforQB-text.tex <==
\section{Blockchain technology}
A blockchain is an architecture that enables data to be stored in a decentralized network \cite{book:Wattenhofer}. The main difference between an traditional database and blockchain is that it allows information to be linked by blocks rather than by relation of the raw data elements. Each block in a blockchain contains some data, the hash of the block itself, and the hash of the previous block. The data stored inside a block depends on the type of blockchain (for example, the Bitcoin blockchain stores transaction details, such as the sender, receiver, and number of coins). Each block also has a hash, which is a fingerprint that identifies the block. It is always unique, calculated once a block is created. Thus, any change inside the block will cause the hash to change. The hash of the previous block contained inside each block allows for creating the ledger or a chain of blocks. \\
Blockchain blocks need not necessarily be in the form of uniform binary data blocks. Modern solutions allow for much richer data structures to be linked \cite{Sopek2022} to form the chain. What is essential is that the entire system represents a consistent generalized transaction history on which all nodes achieve eventual agreement about the linked data.  \\

The main components of blockchain software are consensus and validation algorithms that provide transparency and data security. Unlike ordinary databases, a public blockchain does not rely on centralized model of trust because it is fully available for anyone that wants to participate as a node. Such node gets a full copy of the blockchain and can even use the copy of the blockchain to verify that everything is in order. Therefore the security of a blockchain comes not only from the creative use of encryption, hashing and consensus mechanisms, but also from being distributed and decentralized.\\

Despite the common features of the blockchain software, there are various consensus mechanisms, for example:  Proof of Work (PoW), Proof of Stake (PoS), Delegated Proof of Stake (DPoS), Proof of Authority (PoA), Proof of Capacity (PoC) and many others \cite{Wang2020}. All of them are the mathematical operations through which nodes from the network validate creation of new blocks, however, they differ in the type of algorithm that is used. The most popular and most famous is PoW (used in Bitcoin, early Ethereum and other networks), despite the fact that it needs high computational effort that results in high energy consumption.\\

Regardless of the many advantages of the blockchain, there are huge drawbacks that outcomes from its distributed architecture. In theoretical considerations of distributed systems there are two fundamental theorems that limit desirable properties of blockchain architecture. One of them is known as \textbf{CAP theorem} \cite{Gilbert2012}, the other is \textbf{FLP impossibility result} \cite{FLP}. \\

CAP theorem \cite{Gilbert2012} states any distributed system can have at most two of the following three properties:
\begin{itemize}
\item consistency (C)  --  every read receives the most recent write;
\item availability (A) --  each request eventually receive a response;
\item partition tolerance (P) -- the system operates despite an arbitrary number of messages being dropped between nodes due to communication breakdowns or any other reasons.
\end{itemize}
Unfortunately, the CAP theorem oversimplify the balance between these properties. Due to that this formulation is not genuinely true. CAP theorem states only that perfect availability and consistency in the presence of partitions is not possible. Therefore the designers of distributed systems does not need to choose between consistency and availability when partitions are present. The goal is rather to find a trade-off between them. \\

The FLP impossibility result \cite{FLP}, named after its authors (Fischer, Lynch and Patterson), comes from consideration on achieving consensus in distributed systems. It shows that in an asynchronous setting, there is no distributed algorithm that always solves the consensus problem, even if only one node of the system is fault. \\

The limits ensuing from both CAP and FLP theorems translate to the phenomenon called the \textbf{blockchain trilemma}: \textit{it is impossible for any classical blockchain to simultaneously guarantee security, scalability and decentralization}. Various blockchain consensus algorithms attempted to find a balance between these three features, resembling the trade-offs made by the designers of standard distributed systems. One of the approaches to minimize the negative effects of the trilemma is to prioritize data availability (i.e. scalability) and agree that the data may not be consistent on all nodes at the same time, but to demand that it is eventually consistent, i.e. after some time of the system life.\\   

Since these problems are crucial for the blockchain technology, it is important to analyse new proposals and test new algorithms. Luckily, recent works \cite{Marcozzi2021} shows that the use of quantum mechanical laws and mechanisms can be beneficial for reduction of negative consequence of the trilemma and could lead to entirely new class of blockchain architectures. \\

However, at the same time the emerging quantum computers pose a threat to  the security of modern blockchains, which are built mostly as P2P networks and assume heavy use of the classical asymmetric cryptography with public-private keys playing a pivotal role. Therefore, it is wise to explore the possibilities of integration of quantum cryptography and quantum devices in the blockchain architecture. \\


==> archive/separate-text-inputs/CKAforQB-text1.tex <==
\subsection*{Quantum secured blockchain}
As it was mentioned earlier, the quantum computers pose a threat to any classical encryption algorithms that are used nowadays. Therefore, blockchain protection with quantum cryptography is a sensible step in further development of this technology. \\

This development may take many different paths. 
\begin{itemize}
\item One is to use simply the quantum random number generator for creating the encryption keys. Since such keys have higher degree of randomness than generated using any available algorithms, or obtained using any classical physical processes, this way of communication is a way more secure than the communication that is currently provided.

\item The second is the use of quantum key distribution (QKD) devices that are available on the market and setting quantum channels between each node of the blockchain network (one to one architecture). The use of these devices for obtaining consensus significantly increases the security and ensures the validity of a newly created blocks. Also, as shown in Ref. \cite{Sun2019}, another type of consensus mechanism can be used, which, by using one-time pad encryption keys further improves the security of the blockchain.

\item The third method is to explore different quantum communication protocols that enable the use of other network architectures and favorably affect scalability of such network.

\end{itemize}

The third development path offers the novelty the most therefore, in particular, it is elaborated further in this work. \\


==> archive/separate-text-inputs/CKAforQB-text2.tex <==
\section{Quantum Key Distribution}
Similarly to classical way of data encryption, quantum cryptography also bases on key distribution. The difference here is that the key is generated by non-deterministic purely random process. This process, which occurs in consistence with quantum mechanical laws, secures the distribution of a key itself. For example, since quantum state collapses when measured, the eavesdropping of transmission can be easily detected. Also, due to no-cloning theorem \cite{Wooters1982}, it is impossible to copy the data that is encoded in a quantum state. All of this makes quantum key distribution (QKD) \textit{an information-theoretically secure} solution to the key exchange problem. \\

There are many protocols used for QKD. One of the best known is BB84 \cite{BB84}, named after  Charles Bennett and Gilles Brassard whose presented it in 1984. In this protocol secret key is encoded in photons' polarization states, randomly chosen from two available basis. Each photon represents a single bit of data. Its value is established after the transmission of a photon through the quantum channel and the measurement of its polarization state. Since the measurement is done in two basis, that are also randomly chosen, the outcome of the measurements need to be reconciled by communicating parties. It is done through classical channel (such as phone, mail or any other similar way of communication). Unfortunately, due to that, in the worst case, half of sent bits may need to be removed from the key. Moreover there are also other losses, decoherence and measurement imperfections that may influence the rate of established key. \\

Furthermore, the standard QKD protocols such as that presented above requires to set the quantum channels between all communicating parties. It means that for N parties it is needed to have $\frac{N(N-1)}{2}$ connections. \\

All of this, combined with the high cost of available QKD systems, results in slowdown in development of the commercial use-cases of quantum cryptography. \\
Fortunately, there is novel QKD protocol that allows to decrease the number of connections in the system to N for N communicating parties. It is called Quantum Conference Key Agreement (CKA). \\

==> archive/separate-text-inputs/CKAforQB-text3.tex <==
\section{Quantum distributed consensus algorithm and FLP impossibility}

As it was mentioned earlier, the \textbf{GHZ state} is one of the quantum mechanical tools that enables to achieve distributed consensus \cite{Marcozzi2021, Hondt2004}. In general, GHZ state is an ensemble of N entangled qubits, which state may be mathematically written as
\begin{equation*}
|GHZ\rangle=\frac{1}{\sqrt{2}}\Big(|0\rangle^{\otimes N} + |1\rangle^{\otimes N} \Big) \; .
\end{equation*}
Similarly to the experiment present in previous section, each node in a network receives a single qubit and measures it, choosing "0" if measured state is $|0\rangle$ and 1 otherwise. Due to that the single measurement causes collapse of qubit state to $|0\rangle$ or $|1\rangle$ for each participant of communication, not only those who made the measurement, this allows for obtaining a consensus on single bit of information between multiple nodes. \\

Scheme of a protocol that allows to obtain the consensus over the block of data may look as followed: 
\begin{enumerate}
\item all nodes shares two random, but same bits, $b_1$ and $b_2$;
\item all nodes perform calculation: $b_1\; XOR\; b_2 = b_3$; 
\item all nodes share $b_3$ with others; \\
a) nodes with same value of $b_3$ (the majority) performs an operation on a data block $d_1$:  $b_1 \;XOR \;d_1 = d_2$ (or $b_2 \;XOR \;d_1 = d_2$); \\
b) nodes with different value of $b_3$ do nothing (they are temporarily excluded from adding data to the blockchain); 
\item nodes share $d_2$ with others, if the value is the same they obtain an agreement on data block $d_1$; 
\item the sequence 1-5 is repeated.
\end{enumerate}

It should be noted here, that only the first step of a protocol requires access to the quantum channel (bits $b_1$ and $b_2$ come from the measurement of a quantum state that is shared between parties). All other steps are performed using classical communication layers. \\

Presented method of obtaining consensus provides all properties of distributed consensus \cite{Wang2020, FLP}:
\begin{itemize}
\item agreement -- provided by quantum mechanics (measurement of any entangled qubit cause all other qubits to collapse into an identical state);
\item validity -- provided by proposing either "0" or "1" after the measurement done by first node;
\item wait-free processing -- provided by the entanglement, i.e. the quantum state of all qubits collapses simultaneously.
\end{itemize}
It is worth to mention that faulty nodes do not influence achievement of the consensus, because the consensus is obtained after any measurement performed by any node. \\

Summarizing, the use of GHZ state enables to achieve the consensus in distributed systems and, what is more, overcome FLP impossibility result. \\




==> archive/separate-text-inputs/CKAforQB-text4.tex <==
\section{Further work}
All information above provide a conclusion that development of blockchain technology should take benefits from the law of quantum mechanics. Therefore it is important to not only switch the type of communication between classical and quantum one, but also to investigate novel models of consensus algorithms, reflecting, among other challenges the topologies and architectures of the quantum networks. \\
For this reason, despite the fact it needs some amendments for the use in commercial products, CKA protocol may be interesting solution to the consensus problem in distributed systems. Especially, as shown above, if it solves the FLP impossibility result problem. \\
